Syntax Evolution: Problems and Recursion

To investigate the evolution of syntax, we need to ascertain the evolutionary r\^ole of syntax and, before that, the very nature of syntax. Here, we will assume that syntax is computing. And then, since we are computationally Turing complete, we meet an evolutionary anomaly, the anomaly of sytax: we are syntactically too competent for syntax. Assuming that problem solving is computing, and realizing that the evolutionary advantage of Turing completeness is full problem solving and not syntactic proficiency, we explain the anomaly of syntax by postulating that syntax and problem solving co-evolved in humans towards Turing completeness. Examining the requirements that full problem solving impose on language, we find firstly that semantics is not sufficient and that syntax is necessary to represent problems. Our final conclusion is that full problem solving requires a functional semantics on an infinite tree-structured syntax. Besides these results, the introduction of Turing completeness and problem solving to explain the evolution of syntax should help us to fit the evolution of language within the evolution of cognition, giving us some new clues to understand the elusive relation between language and thinking.

==> fonts.tex <==
% FONTS.TEX (RMCG19940923)

\catcode`\@=11

% Adaptado de pdcfsel.tex (v 3.5, 1995/03/28) by P. Damian Cugley

\def\expcs#1#2{\expandafter#1\csname#2\endcsname}
\def\noexpcs{\expcs\noexpand}

\def\loadfont#1#2{\ifx#1\relax \FSELloadfont#1{#2}\else
 \ifx#1\UNDEFINED \FSELloadfont#1{#2}\fi\fi}

\def\FSELloadfont#1#2{\edef#1{\global\font\noexpand#1#2\relax\noexpand#1}}

\def\xfontset#1#2#3{
    \def\f##1##2{\expcs\loadfont{#1##1}{##2#3}}
    \let\m=\f \let\M=\f
    \def\@##1##2##3{\expcs\loadfont{#1##2}{##3 at #3pt }}
    #2 }

\def\fontset#1#2#3#4#5#6{\xfontset{#1}{#2}{#3}%
    \expcs\edef{#1fonts}{%
       \noexpcs{#1mathsfonts}%
       \noexpand\FSELnicknames{#1}{#5}{#6}\noexpand#2%
       \noexpand\setbaselineskip{#4}%
       \noexpand\rm }%
       \expcs\def{#1mathsfonts}{\FSELloadmaths{#1}{#5}{#6}#2}}

\def\FSELnicknames#1#2#3{\let\@\relax
    \def\f##1##2{\expcs\edef{##1}{\noexpcs{#1##1}}}%
    \def\m##1##2{%
       \expcs\textfont{##1fam}\csname#1##1\endcsname
       \expcs\scriptfont{##1fam}\csname#2##1\endcsname
       \expcs\edef{##1}{%
           \fam\expcs\noexpand{##1fam}%
           \expcs\noexpand{#1##1}}}%
    \def\M##1{\expcs\scriptscriptfont{##1fam}\csname#3##1\endcsname
       \m{##1}}}

\def\setbaselineskip#1{\ifdim #1=\baselineskip \else
    \baselineskip#1\relax \normalbaselineskip\baselineskip
    \jot0.25\baselineskip
    \smallskipamount 0.25\baselineskip plus 0.083\baselineskip
       minus 0.083\baselineskip
    \medskipamount 0.5\baselineskip plus 0.167\baselineskip
       minus 0.167\baselineskip
    \bigskipamount 1\baselineskip plus 0.333\baselineskip
       minus 0.333\baselineskip
    \setbox\strutbox=\hbox{\vrule height 0.708\baselineskip
       depth 0.292\baselineskip width\z@}%
    \def\big##1{{\hbox{$\left##1\vbox to0.708\baselineskip
       {}\right.\n@space$}}}%
    \def\Big##1{{\hbox{$\left##1\vbox to0.958\baselineskip
       {}\right.\n@space$}}}%
    \def\bigg##1{{\hbox{$\left##1\vbox to1.208\baselineskip
       {}\right.\n@space$}}}%
    \def\Bigg##1{{\hbox{$\left##1\vbox to1.458\baselineskip
       {}\right.\n@space$}}}%
    \topskip=0.833\baselineskip \splittopskip=\topskip
    \abovedisplayskip=1\baselineskip
       plus0.25\baselineskip minus0.75\baselineskip
    \abovedisplayshortskip=0pt plus0.25\baselineskip
    \belowdisplayskip=\abovedisplayskip
    \belowdisplayshortskip=0.583\baselineskip
       plus0.25\baselineskip minus0.333\baselineskip
 \fi}

\def\FSELloadmaths#1#2#3{%
    \let\@\relax \def\f##1##2{}%
    \def\m##1##2{\csname#1##1\endcsname \csname#2##1\endcsname}%
    \def\M##1{\csname#3##1\endcsname \m{##1}}%
    \global\expcs\let{#1mathsfonts}\relax}

\chardef\rmfam=0 \chardef\mifam=1 \chardef\syfam=2

% Databases

\def\cmtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\xfontset{cmscriptscript}\cmtemplate{5}
\xfontset{cmscript}\cmtemplate{7}
\fontset{cm}\cmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\def\viiitemplate{%
   \m{rm}{cmr}\f{it}{cmti}\m{bf}{cmbx}%
   \f{sl}{cmsl}\f{tt}{cmtt}\m{mi}{cmmi}\m{sy}{cmsy}}
\xfontset{viiiscript}\viiitemplate{6}
\fontset{viii}\viiitemplate{8}{10pt}{viiiscript}{viiiscript}

\def\xiitemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xiisc{cmcsc10 at 12pt }
\loadfont\xiisy{cmsy10 at 12pt }
\xfontset{xiiscriptscript}\xiitemplate{6}
\xfontset{xiiscript}\xiitemplate{9}
\fontset{xii}\xiitemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}

\def\xiibtemplate{%
   \M{rm}{cmr}\@\m{it}{cmbxti10}\M{bf}{cmbx}\@\f{sc}{cmssbx12}%
   \@\f{sl}{cmbxsl10}\@\f{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xiibscriptscript}\xiibtemplate{6}
\xfontset{xiibscript}\xiibtemplate{9}
\fontset{xiib}\xiibtemplate{12}{14.4pt}{xiibscript}{xiibscript}

\def\xivtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \m{sl}{cmsl}\m{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xivrm{cmr12 at 14.4pt }
\loadfont\xivit{cmti12 at 14.4pt }
\loadfont\xivbf{cmbx12 at 14.4pt }
\loadfont\xivsc{cmcsc10 at 14.4pt }
\loadfont\xivsl{cmsl12 at 14.4pt }
\loadfont\xivtt{cmtt12 at 14.4pt }
\loadfont\xivmi{cmmi12 at 14.4pt }
\loadfont\xivsy{cmsy10 at 14.4pt }
\xfontset{xivscript}\xivtemplate{10}
\xfontset{xivscriptscript}\xivtemplate{7}
\fontset{xiv}\xivtemplate{14.28}{17pt}{xivscript}{xivscriptscript}

\def\xivbtemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmbxti10}\@\m{bf}{cmbx12}\@\f{sc}{cmr12}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xivbscript}\xivbtemplate{7}
\fontset{xivb}\xivbtemplate{14.28}{17pt}{xivbscript}{xivbscript}

\def\xviitemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmti12}\@\m{bf}{cmbx12}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\@\m{mi}{cmmi12}\@\m{sy}{cmsy10}}
\xfontset{xviiscript}\xviitemplate{12}
\fontset{xvii}\xviitemplate{17.28}{21pt}{xviiscript}{xviiscript}

\def\xviibtemplate{%
   \@\m{rm}{cmbx12}\@\m{it}{cmbxti10}\@\m{bf}{cmbx12}\@\f{sc}{cmr17}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xviibscript}\xviibtemplate{12}
\fontset{xviib}\xviibtemplate{17.28}{21pt}{xviibscript}{xviibscript}

\def\xxitemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmti12}\@\m{bf}{cmbx12}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\@\m{mi}{cmmi12}\@\m{sy}{cmsy10}}
\xfontset{xxiscript}\xxitemplate{14.28}
\fontset{xxi}\xxitemplate{20.736}{25pt}{xxiscript}{xxiscript}

\def\lmtemplate{%
   \M{rm}{texnansi-lmr}\m{it}{texnansi-lmri}%
   \M{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\M{mi}{cmmi}\M{sy}{cmsy}}
\fontset{lm}\lmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\loadfont\lmxiisy{cmsy10 at 12pt }
\fontset{lmxii}\lmtemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}
\fontset{lmix}\lmtemplate{9}{11pt}{cmscript}{cmscriptscript}

\def\lmviiitemplate{%
   \m{rm}{texnansi-lmr}\f{it}{texnansi-lmri}%
   \m{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\m{mi}{cmmi}\m{sy}{cmsy}}
\fontset{lmviii}\lmviiitemplate{8}{10pt}{viiiscript}{viiiscript}

\loadfont\lmxiizero{texnansi-lmr17 at 21pt }
\loadfont\lmxiione{texnansi-lmbx12 at 17pt }
\loadfont\lmxiitwo{texnansi-lmbx12 at 14.4pt }
\loadfont\lmzero{texnansi-lmr17}
\loadfont\lmone{texnansi-lmbx12 at 14.4pt }
\loadfont\lmtwo{texnansi-lmbx12}
\def\lmtitles{\def\fontzero{\lmzero}%
 \def\fontone{\lmone}\def\fonttwo{\lmtwo}}
\def\lmxiititles{\def\fontzero{\lmxiizero}%
 \def\fontone{\lmxiione}\def\fonttwo{\lmxiitwo}}

\def\pstemplate{%
   \@\M{rm}{ptmr8r}\@\M{it}{ptmri8r}\@\M{bf}{ptmb8r}\@\f{sc}{ptmrc8t}%
   \@\M{mi}{ptmri8t}\@\M{tt}{pcrr8r}}
\xfontset{psxscriptscript}\pstemplate{5}
\xfontset{psxscript}\pstemplate{7}
\fontset{psx}\pstemplate{10}{12pt}{psxscript}{psxscriptscript}

\xfontset{psxiiscriptscript}\pstemplate{6}
\xfontset{psxiiscript}\pstemplate{9}
\fontset{psxii}\pstemplate{12}{14.4pt}{psxiiscript}{psxiiscriptscript}

\xfontset{psxivscriptscript}\pstemplate{7}
\xfontset{psxivscript}\pstemplate{11}
\fontset{psxiv}\pstemplate{14.4}{17.28pt}{psxivscript}{psxivscriptscript}

\xfontset{psxviiscriptscript}\pstemplate{9}
\xfontset{psxviiscript}\pstemplate{14}
\fontset{psxvii}\pstemplate{17}{21pt}{psxviiscript}{psxviiscriptscript}

\xfontset{psxxiscriptscript}\pstemplate{10}
\xfontset{psxxiscript}\pstemplate{14}
\fontset{psxxi}\pstemplate{21}{25pt}{psxxiscript}{psxxiscriptscript}

\def\zerotemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\M{sl}{cmsl}%
   \M{tt}{cmtt}}
\loadfont\zerobf{cmbx12 at 17.28pt }
\loadfont\zeroit{cmti12 at 17.28pt }
\loadfont\zerosl{cmsl12 at 17.28pt }
\loadfont\zerott{cmtt12 at 17.28pt }
\xfontset{zeroscriptscript}\zerotemplate{9}
\xfontset{zeroscript}\zerotemplate{12}
\fontset{zero}\zerotemplate{17}{20.4pt}{zeroscript}{zeroscriptscript}

\def\onetemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\m{sl}{cmsl}%
   \m{tt}{cmtt}}
\loadfont\onerm{cmr12 at 14.4pt }
\loadfont\onebf{cmbx12 at 14.4pt }
\loadfont\oneit{cmti12 at 14.4pt }
\loadfont\onesl{cmsl12 at 14.4pt }
\loadfont\onett{cmtt12 at 14.4pt }
\xfontset{onescriptscript}\onetemplate{7}
\xfontset{onescript}\onetemplate{10}
\fontset{one}\onetemplate{14.4}{17.28pt}{onescript}{onescriptscript}

% Fonts for titles

\def\cmtitles{%
 \def\fontzero{\xviifonts\rm}%
 \def\fontone{\xivfonts\bf}%
 \def\fonttwo{\xiifonts\bf}%
}
\def\viiititles{%
 \def\fontzero{\xivfonts\bf}%
 \def\fontone{\xiifonts\bf}%
 \def\fonttwo{\cmfonts\bf}%
}
\def\xiititles{%
 \def\fontzero{\xxifonts\rm}%
 \def\fontone{\xviibfonts\bf}%
 \def\fonttwo{\xivbfonts\bf}%
 \def\fontthree{\xiibfonts\bf}%
}
\def\psxtitles{%
 \def\fontzero{\psxviifonts\rm}%
 \def\fontone{\psxivfonts\bf}%
 \def\fonttwo{\psxiifonts\bf}%
}
\def\psxiititles{%
 \def\fontzero{\psxxifonts\rm}%
 \def\fontone{\psxviifonts\bf}%
 \def\fonttwo{\psxivfonts\bf}%
}
\cmtitles

\catcode`\@=12

\endinput


==> index.tex <==
% index.tex (RMCG19931103)

\catcode`\@=11

\catcode`\^^02=12 \catcode`\^^03=12 \catcode`\^^04=12 \catcode`\^^05=12

% Check files auxiliar.aux, auxiliar.ind

\newread\infile

\newif\ifauxf
\openin\infile=auxiliar.aux
\ifeof\infile \auxffalse \else \auxftrue \fi
\closein\infile

\newif\ifindf
\openin\infile=auxiliar.ind
\ifeof\infile \indffalse \else \indftrue \fi
\closein\infile

% pdftex

\ifx\pdfoutput\undefined \csname newcount\endcsname\pdfoutput \fi

% \color{Red} ... \endcolor

\def\cmykWhite{0 0 0 0} \def\cmykDarkWhite{0 0 0 .3}
\def\cmykGray{0 0 0 .5} \def\cmykDarkGray{0 0 0 .7}
\def\cmykBlack{0 0 0 1} \def\cmykDarkBlack{.4 .3 .3 1}
\def\cmykYellow{0 0 1 0} \def\cmykDarkYellow{0 0 1 .7}
\def\cmykMagenta{0 1 0 0} \def\cmykDarkMagenta{0 1 0 .7}
\def\cmykCyan{1 0 0 0} \def\cmykDarkCyan{1 0 0 .7}
\def\cmykRed{0 1 1 0} \def\cmykDarkRed{0 1 1 .7}
\def\cmykGreen{1 0 1 0} \def\cmykDarkGreen{1 0 1 .7}
\def\cmykBlue{1 1 0 0} \def\cmykDarkBlue{1 1 0 .7}

\newcount\col@rstack
\def\pdf@color#1{\pdfcolorstack\col@rstack push {\csname cmyk#1\endcsname k}}
 \def\pdf@darkcolor#1{\pdfcolorstack\col@rstack push {\csname cmykDark#1\endcsname k}}
 \def\pdf@endcolor{\pdfcolorstack\col@rstack pop}
 \def\pdf@black{\pdfcolorstack\col@rstack push {0 g}}
\def\dvips@color#1{\special{color push cmyk \csname cmyk#1\endcsname}}
 \def\dvips@darkcolor#1{\special{color push cmyk \csname cmykDark#1\endcsname}}
 \def\dvips@endcolor{\special{color pop}}
 \def\dvips@black{\special{color push gray 0}}
\def\dvipdf@color#1{\special{pdf: bc [\csname cmyk#1\endcsname]}}
 \def\dvipdf@darkcolor#1{\special{pdf: bc [\csname cmykDark#1\endcsname]}}
 \def\dvipdf@endcolor{\special{pdf: ec}}
 \def\dvipdf@black{\special{pdf: bc [0]}}

\ifcase\pdfoutput
 \ifx\dvips\undefined
  \special{pdf: sc [0]}\let\colorblack=\dvipdf@black
  \def\colors{\let\color=\dvipdf@color\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
  \def\darkcolors{\let\color=\dvipdf@darkcolor\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
 \else
  \special{color gray 0}\let\colorblack=\dvips@black
  \def\colors{\let\color=\dvips@color\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
  \def\darkcolors{\let\color=\dvips@darkcolor\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
 \fi
\else
 \col@rstack=\pdfcolorstackinit page {0 g}\let\colorblack=\pdf@black
 \def\colors{\let\color=\pdf@color\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
 \def\darkcolors{\let\color=\pdf@darkcolor\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
\fi

\def\nocolor{\def\color##1{\relax}\def\truecolor##1{\relax}\def\endcolor{\relax}}
\nocolor % default value, \darkcolors intermediate with \colors

% type of links

\def\numlink#1{num \number#1}
\def\namelink#1{name {(\number#1)}}
\ifx\xmpinclude\undefined \let\typelink=\numlink \else \let\typelink=\namelink \fi

% \goto{Text in red}{123}

{\catcode`\#=12 \xdef\hash{#}}

\def\pdf@goto#1#2{\leavevmode
 \pdfstartlink attr{/F 4 /Border [0 0 0]} goto \typelink{#2}%
 \color{Red}#1\endcolor\pdfendlink\relax}
\def\dvips@goto#1#2{\leavevmode
 \special{html:<a href=\string"\hash\typelink{#2}\string">}%
 \color{Red}#1\endcolor\special{html:</a>}\relax}
\def\dvipdf@goto#1#2{\leavevmode
 \special{pdf: bann << /Type /Annot /Subtype /Link /Border [0 0 0]
   /A << /S /GoTo /D (\typelink{#2}) >> >>}\color{Red}#1\endcolor
 \special{pdf: eann}\relax}
\def\nolinks@goto#1#2{\leavevmode
 \closeout-1\color{Red}#1\endcolor\closeout-1\relax}
%\closeout-1 is just a whatsit, i.e. an extension as pdf commands are

% \dest

\newcount\d@stno

\def\pdf@dest{\global\advance\d@stno1
 \ifvmode \pdfdest \typelink{\d@stno} fitbh\else
  \vbox to0pt{\vss\pdfdest \typelink{\d@stno} fitbh\kern1pc}\fi}
\def\dvips@dest{\global\advance\d@stno1
 \ifvmode \special{html:<a name=\string"\typelink{\d@stno}\string">}
          \special{html:</a>}\else
  \vbox to0pt{\vss\special{html:<a name=\string"\typelink{\d@stno}\string">}
                  \special{html:</a>}\kern1pc}\fi}
\def\dvipdf@dest{\global\advance\d@stno1
 \ifvmode
  \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\else
  \vbox to0pt{\vss
   \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\kern1pc}\fi}
\def\nolinks@dest{\global\advance\d@stno1
 \ifvmode \closeout-1\else \vbox to0pt{\vss\closeout-1\kern1pc}\fi}

\ifcase\pdfoutput
 %\def\pdfcode#1\pdfendcode{\relax\closeout-1\relax}
 \ifx\dvips\undefined
  \def\links{\let\goto=\dvipdf@goto\let\dest=\dvipdf@dest}
 \else
  \def\links{\let\goto=\dvips@goto\let\dest=\dvips@dest}
 \fi
\else
 %\let\pdfcode=\relax \let\pdfendcode=\relax
 \def\links{\let\goto=\pdf@goto\let\dest=\pdf@dest}
\fi

\def\nolinks{\let\goto=\nolinks@goto\let\dest=\noliks@dest}
\links % default value

% \footnote

\def\footnoteoptions{} % \eightpt, for example
% adapted from [363]; parameter #2 (the text) is read later
\def\footnote#1{\let\@sf\empty
  \ifhmode\edef\@sf{\spacefactor\the\spacefactor}\/\fi
  \global\advance\d@stno1 \goto{#1}{\number\d@stno}\global\advance\d@stno-1% RMCG
  \@sf\vfootnote{#1}}
\def\vfootnote#1{\insert\footins\bgroup
  \interlinepenalty\interfootnotelinepenalty
  \splittopskip\ht\strutbox % top baseline for broken footnotes
  \splitmaxdepth\dp\strutbox \floatingpenalty\@MM
  \leftskip\z@skip \rightskip\z@skip \spaceskip\z@skip \xspaceskip\z@skip
  \footnoteoptions \textindent{#1}\footstrut\dest\futurelet\next\fo@t} % RMCG

% \pdf@ut calculates the number of branches in \@utno

\newtoks\pdft@k \pdft@k{}
\def\pdft@toc#1{\global\pdft@k=\expandafter{\the\pdft@k#1}}
\newcount\@utno \newcount\@uts
\newcount\@utss \newcount\@utt
\def\c@rcdr#1#2,{\edef\car{#1}\edef\cdr{#2}\ifx\cdr\empty\edef\cdr{0}\fi}
\def\pdf@ut{\expandafter\c@rcdr\the\pdft@k,\@uts=\car
 \global\pdft@k=\expandafter{\cdr}\toks0=\expandafter{\cdr}%
 \@utno=0 \@utss=\car \advance\@utss1
 \loop \expandafter\c@rcdr\the\toks0,\@utt=\car\toks0=\expandafter{\cdr}%
  \ifnum\@uts<\@utt \ifnum\@utss=\@utt\advance\@utno1\fi \repeat}

% Indexing

\def\ref#1{??} \def\refsc#1{??} \def\refpg#1{??} \def\refx#1#2{??}
% \toc{level}{text} \pdftocline{text}{\d@stno}
\let\toc=\gobbletwo \let\pdftocline=\gobbletwo
% \lbl{mnemonic}{replacement} \ndx{text}{type}
\let\lbl=\gobbletwo \let\ndx=\gobbletwo

% \pdfout{level}{title}{secid}
\def\pdfout#1#2#3{\if*#3#2\else#3 #2\fi}
\def\pdfoutA#1#2#3{#3 #2}
\def\pdfoutB#1#2#3{#2}

\catcode`\(=13 \catcode`\)=13
 \def({\string\(} \def){\string\)}
\catcode`\(=12 \catcode`\)=12

\def\pdf@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
  {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
   \pdfoutline goto \typelink{#3} count \number\@utno
               {\pdfout{#1}{#2}{#4}}}\fi}
\def\dvips@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
 {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
  \special{ps: [ /Title (\pdfout{#1}{#2}{#4}) /Count \number\@utno\space
   /Page #5 /OUT pdfmark}}\fi}
\def\dvipdf@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
 {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
  \special{pdf: out #1 << /Title (\pdfout{#1}{#2}{#4})
   /Dest (\typelink{#3}) >>}}\fi}

\def\fourdigits#1{\ifnum#1<0 \errmessage{min is 0}\else
            \ifnum#1>9999 \errmessage{max is 9999}\else
 \ifnum#1<1000 0\fi \ifnum#1<100 0\fi \ifnum#1<10 0\fi\fi\fi \number#1}
\ifx\secid\undefined \let\secid\empty\fi

\def\save#1{{\def\\{\string\\}\def~{\string~}\def\S{\string\S}\stringaccents
  \stringate\dohigh \deactivate\dohigh \utf\utf@Ch \let^^c2\empty
  \edef\next{\write\auxf{#1\string{\fourdigits\d@stno\string}%
    \string{\secid\string}\string{\noexpand\folio\string}}}\next}}

\newwrite\auxf \newwrite\tocf \newwrite\ndxf

\def\files{\begingroup \stringate\dohigh\stringaccents \let^^c2\empty
 \def~{\string~}\def\\{\string\\}\def\S{\string\S}\def\&{\string\&}% \catcode`\@=11
 \def\ftoc##1##2##3##4##5{\ifnum##1<9\pdft@toc{##1}\fi
  \immediate\write\tocf{\string\tocline
   \string{##1\string}\string{##2\string}%
   \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\fndx##1##2##3##4##5{\immediate\write\ndxf{\string\ndxline
  \string{##1\string}\string{##2\string}%
  \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\flbl##1##2##3##4##5{\setbox0=\hbox{\csname ^^03##1\endcsname}%
  \ifdim\wd0=0pt
   \expandafter\gdef\csname ^^02##1\endcsname{##2}% replacement
   \expandafter\gdef\csname ^^03##1\endcsname{##3}% \d@stno
   \expandafter\gdef\csname ^^04##1\endcsname{##4}% \secid
   \expandafter\gdef\csname ^^05##1\endcsname{##5}% \folio
  \else\errmessage{label ##1 redefined}\fi}
 \ifauxf
  \immediate\openout\tocf=auxiliar.toc
  \immediate\openout\ndxf=auxiliar.ind
  \input auxiliar.aux
  \immediate\closeout\tocf \immediate\closeout\ndxf
  \def\\{ }\pdft@toc0 \catcode`\(=13 \catcode`\)=13
  \ifcase\pdfoutput
   \ifx\dvips\undefined \let\tocline=\dvipdf@outline
   \else \let\tocline=\dvips@outline\fi
  \else \let\tocline=\pdf@outline \fi
  \input auxiliar.toc
 \fi
 \endgroup
 \openout\auxf=auxiliar.aux
 \def\ref{\r@f^^02}\def\refsc{\r@f^^04}\def\refpg{\r@f^^05}\def\refx{\r@fx}%
 \def\toc##1##2{\save{\string\ftoc\string{##1\string}\string{##2\string}}}%
 \def\lbl##1##2{\save{\string\flbl\string{##1\string}\string{##2\string}}}%
 \def\ndx##1##2{\save{\string\fndx\string{##1\string}\string{##2\string}}}%
}
% Note that \vbox{}someword or someword\vbox{} does not hyphenate someword.

\def\r@f#1#2{{\stringate\dohigh\stringaccents\def\&{\string\&}\utf\utf@Ch \let^^c2\empty
  \xdef\n@@{\string"#2\string" }\xdef\@@n{\csname ^^03#2\endcsname}%
  \expandafter\global\expandafter\let\expandafter\@n@\csname #1#2\endcsname}%
 \setbox0=\hbox{\@n@}\ifdim\wd0=0pt ?\ifauxf\errmessage{label \n@@ undefined}\fi
  \else\goto{\@n@}{\@@n}\fi}

\def\r@fx#1#2{{\stringate\dohigh\stringaccents\def\&{\string\&}\utf\utf@Ch \let^^c2\empty
  \xdef\n@@{\string"#2\string" }\xdef\@@n{\csname ^^03#2\endcsname}}%
 \setbox0=\hbox{\@@n}\ifdim\wd0=0pt ?\ifauxf\errmessage{label \n@@ undefined}\fi
  \else\goto{#1}{\@@n}\fi}

\def\label#1#2{\dest\lbl{#1}{#2}}
\def\index#1#2{\dest\ndx{#1}{#2}}

\catcode`\@=12

